Branch-Train-Merge: Embarrassingly Parallel Training of Expert Language Models

We present Branch-Train-Merge (BTM), a communication-efficient algorithm for embarrassingly parallel training of large language models (LLMs). We show it is possible to independently train subparts of a new class of LLMs on different subsets of the data, eliminating the massive multi-node synchronization currently required to train LLMs. BTM learns a set of independent expert LMs (ELMs), each specialized to a different textual domain, such as scientific or legal text. These ELMs can be added and removed to update data coverage, ensembled to generalize to new domains, or averaged to collapse back to a single LM for efficient inference. New ELMs are learned by branching from (mixtures of) ELMs in the current set, further training the parameters on data for the new domain, and then merging the resulting model back into the set for future use. Experiments show that BTM improves in- and out-of-domain perplexities as compared to GPT-style Transformer LMs, when controlling for training cost. Through extensive analysis, we show that these results are robust to different ELM initialization schemes, but require expert domain specialization; LM ensembles with random data splits do not perform well. We also present a study of scaling BTM into a new corpus of 64 domains (192B whitespace-separated tokens in total); the resulting LM (22.4B total parameters) performs as well as a Transformer LM trained with 2.5 times more compute. These gains grow with the number of domains, suggesting more aggressive parallelism could be used to efficiently train larger models in future work.

==> tables/averaging_across_ratios.tex <==
% \begin{table*}[t]\small
% \centering
% % \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% &  \multicolumn{4}{c}{ \bf GPT-3 Small} \\
% \cmidrule{2-5}
% % % \emph{Shared Params}  & 124M & 124M & 96.1M & 67.8M  \\
% % % \emph{Expert Params}  & 0 & 0 & 28.3M & 56.7M  \\
% % % \emph{Total Params} & 124M & 124M & 322.8M & 521.1M  \\
% % \cmidrule{2-5}

% \textbf{Domain} & \bf \dataparallel  & \bf \domaintoken & \bf \plusmodelayers (L/2) & \bf \plusmodelayers (L) \\ %& \boldmath{\lnot}\textbf{\dapt}\\
% \midrule 

% \oneb 


% % 82.1
% & 14.6 & 14.2 & 14.3 & \bf 13.5  \\ %& 79.0$_{4.1}$\\


% \cs 
% % 82.1
% & 17.9 & 17.8 & 17.0 & \bf 15.6  \\ %& 79.0$_{4.1}$\\


% \legal 
% % 82.1
% & 10.5 & 10.1 &  9.5 & \bf 9.0   \\ %& 79.0$_{4.1}$\\


% \med  
% % 82.1
% & 13.8 & 14.1 & 13.4 & \bf 11.8 \\ %& 79.0$_{4.1}$\\


% \webtext 
% % 82.1
% & 22.0 & \bf 20.5 & 21.8 & 21.1 \\%& 79.0$_{4.1}$\\


% \realnews 
% % 82.1
% & 20.1 & \bf 18.6 & 20.0 &  18.8 \\ %& 79.0$_{4.1}$\\


% \reddit 
% % 82.1
% & 40.9 & \bf 40.3 & 41.6 &  40.8 \\ %& 79.0$_{4.1}$\\


% \reviews 
% % 82.1
% & 23.9 &  23.2 & 22.3 &  \bf 20.5\\ %& 79.0$_{4.1}$\\

% \midrule
% \bf Average & 20.5 & 19.9 &  20.0 & \bf 18.9 \\

% \bottomrule
% \end{tabular}
% % }
% \caption{Conditioning GPT-3 small on domains improves in-domain test performance, when training with 32 GPUs for 48 hours. See Appendix \label{sec:validation_curves} for validation curves during training.} 
% \label{tab:base_results}
% \end{table*}



\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rccccccccccc}
\toprule
& \multicolumn{10}{c}{\bf Seed Phase (125M Parameter Model / Expert)}\\
& 0\% & 10\% & 20\% & 30\% & 40\% & 50\% & 60\% & 70\% & 80\% & 90\% & 100\%\\
\cmidrule{2-12}
\bf Train Domains    & 283.9 & 23.4 &  18.5 &  18.3 & 18.1     & \bf 18.0 & \bf 18.0 & 18.2       & 18.6 & 19.0 & 19.8 \\
\bf Eval Domains       & 278.1  & 79.3 & 44.7    & 34.2     & 31.2     & 28.5 & 25.8 & 24.7   & \bf 24.6 & 24.8 & 25.5  \\
\bf Avg                 & 281.0  & 51.4 & 31.6     & 26.2    & 24.7 & 23.3 & 21.9  & \bf 21.4       & 21.6 & 21.9 & 22.7\\

\midrule
\end{tabular}

\begin{tabular}{rccccccccc}
% \midrule
& \multicolumn{9}{c}{\bf Seed Phase (350M Parameter Model / Expert)}\\
& 0\% & 12.5\% & 25\% & 37.5\% & 50\% & 62.5\% & 75\% & 87.5\% & 100\%\\
% &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-10}
\bf Train Domains & 77.9 & 18.7   & 15.4   &  15.3   & \bf 15.1    & \bf 15.1  & 15.5  & 15.9  & 16.3 \\
\bf Eval Domains & 1755.2  & 30.8   & 24.2   & 21.9  & 20.4    & 20.3  & 20.2   & \bf 20.1   &  20.8 \\
\bf Avg & 916.5 & 24.8   & 19.8  &  18.6    &  \bf 17.7   & \bf 17.7   & 17.8  & 18.0 & 18.5\\
\bottomrule\\

\end{tabular}
% \begin{tabular}{rccccccccccccccccc}
% \toprule
% & \multicolumn{13}{c}{\bf Dense Phase (350M Parameter Model / Experts)}\\
% % & 0\% & 10\% & 20\% & 30\% & 40\% & 50\% & 60\% & 70\% & 80\% & 90\% & 100\%\\
% % &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
% \cmidrule{2-16}
% \bf Training Domains & 15.3 & 15.1 & 15.0   & 14.8 & 14.9   & \bf 14.7  & \bf 14.7  & \bf 14.7  & \bf 14.7    & 14.8  & 14.9  & 15.0  & x  & 15.4  & 15.7  & 15.7 & 16.3 \\
% \bf Novel Domains & 21.3 & 20.9 & 20.0  & 19.7  & 19.6  & 19.2  & 19.0  & 18.7  & 18.6    & 18.5    & \bf 18.4  & 18.6  & x   & 19.2  & 19.4  & 19.4 & 20.8 \\
% \bf Avg & 18.3 & 18.0   & 17.5  & 17.3  & 17.2  & 17.0  & 16.9  & 16.7  & 16.7  & \bf 16.6    & 16.7  & 16.8  & x   & 17.3  & 17.5  & 17.6  & 18.5\\
% \bottomrule
% \end{tabular}

% }
\caption{Average test perplexity on train and eval domain test sets when averaging \dslm{}s with different seed phase budgets for the 125M and 350M parameter LMs. Lowest perplexity is achieved at slightly higher seed phase training proportions than when ensembling; however, the change in performance is small throughout the 20-80\% range. These results are also visualized in Figure~\ref{fig:averaging_across_ratios}.}
\label{tab:averaging_across_ratios}
\end{table}


==> tables/averaging_results_all.tex <==
\begin{table}[t]\small
\centering
% \begin{subtable}[t]{0.3\textwidth}

\begin{subtable}[t]{0.48\textwidth}
\begin{tabular}{rcccc}
\toprule
\multicolumn{5}{l}{\textbf{125M}} \\ %(16 GPUs -- 80k updates)} \\
\cmidrule{1-4}
 \denselm & \delm Avg & \delm Avg & \delm Avg & \delm Ensemble \\
& & 125M & 125M & 125M & 1B \\

& 125M & 512M & 125M & 1B \\
\cmidrule{2-4}
Train   & 19.9$_{0.23}$    & 18.2$_{0.82}$  & \bf 17.2$_{0.02}$ \\
Eval   & 25.2$_{0.18}$    & 23.4$_{0.54}$  & \bf 22.4$_{0.12}$ \\
All     & 22.5$_{0.14}$    & 20.8$_{0.63}$  & \bf 19.8$_{0.05}$ \\
\end{tabular}
\end{subtable}
\hfill
\begin{subtable}[t]{0.48\textwidth}
\begin{tabular}{rccc}
% \multicolumn{5}{c}{350M}
\toprule
\multicolumn{4}{l}{\bf 350M} \\ %(32 GPUs -- 32k updates)} \\
\cmidrule{1-4}
& \denselm & \demix &  \delm\\
& 350M & 1.8B & 2.8B \\
\cmidrule{2-4}
Train     &  16.3   & 15.0      &  \bf 14.7 \\
Eval     &  20.8   & 19.9      & \bf 18.6\\
All      & 18.5     & 17.5      &  \bf 16.7 \\
\end{tabular}
\end{subtable}

\begin{subtable}[t]{0.48\textwidth}
\begin{tabular}{rccc}
% \multicolumn{5}{c}{750M}
\toprule
\multicolumn{4}{l}{\bf 750M} \\ %(64 GPUs -- 24k updates)} \\
\cmidrule{1-4}
& \denselm & \demix & \delm\\
& 750M & 3.8B  & 6B \\
\cmidrule{2-4}
% \parbox[t]{3pt}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\bf {\textsc{750M}}}}} &
% \parbox[t]{3pt}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\bf {\textsc{64 GPUs}}}}} 
Train   & 14.7      & 13.5	    & \bf 13.4  \\
Eval   & 19.3      & 17.7      & \bf 16.7  \\
All     & 17.0      & 15.6      & \bf 15.0 \\
\bottomrule \\
\end{tabular}
\end{subtable}
\hfill
\begin{subtable}[t]{0.48\textwidth}
\begin{tabular}{rccc}
% \multicolumn{6}{c}{1.3B}
\toprule
\multicolumn{4}{l}{\textbf{1.3B}} \\ %(128 GPUs -- 12k updates)} \\
\cmidrule{1-4}
& \denselm & \demix & \delm\\
& 1.3B & 7B & 10.4B \\
\cmidrule{2-4}
Train   & 14.2      & 13.7      & \bf 13.0  \\
Eval   & 18.4      & 17.6      & \bf 16.3 \\
All     & 16.3      & 15.6      & \bf 14.6  \\
\bottomrule \\
\end{tabular}
\end{subtable}

% \begin{tabular}{rcccc}
% \toprule
% \multicolumn{5}{l}{\bf 125M -- 16 GPUs -- 80k updates} \\
% \cmidrule{1-5}
% & \dense & \demix & \modular  & \densetomod \\
% & 125M & 512M & 1B  & 1B \\
% \cmidrule{2-5}
% Train   & 19.9$_{0.23}$    & 18.2$_{0.82}$    & 18.0$_{0.48}$    & \bf 17.2$_{0.02}$ \\
% Novel   & 25.2$_{0.18}$    & 23.4$_{0.54}$    & 24.1$_{0.49}$    & \bf 22.4$_{0.12}$ \\
% All     & 22.5$_{0.14}$    & 20.8$_{0.63}$    & 21.0$_{0.33}$    & \bf 19.8$_{0.05}$ \\
% \end{tabular}
% % \end{subtable}

% % \begin{subtable}[t]{0.3\textwidth}
% \begin{tabular}{rcccc}
% % \multicolumn{5}{c}{350M}
% \midrule
% \multicolumn{5}{l}{\bf 350M -- 32 GPUs -- 32k updates} \\
% \cmidrule{1-5}
% & \dense & \demix & \modular  & \densetomod \\
% & 350M & 1.8B & 2.8B  & 2.8B \\
% \cmidrule{2-5}
% Train     &  16.3    &   15.0  &  15.3         &  \bf 14.7 \\
% Novel      &  20.8      &     19.9      &    21.3      & \bf 18.6\\
% All      & 18.5    &    17.5  &  18.3     &  \bf 16.7 \\
% \end{tabular}
% % \end{subtable}

% \begin{tabular}{rcccc}
% % \multicolumn{5}{c}{750M}
% \midrule
% \multicolumn{5}{l}{\bf 750M -- 64 GPUs -- 24k updates} \\
% \cmidrule{1-5}
% & \dense & \demix & \modular  & \densetomod \\
% & 750M & 3.8B  & 6B  & 6B \\
% \cmidrule{2-5}
% % \parbox[t]{3pt}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\bf {\textsc{750M}}}}} &
% % \parbox[t]{3pt}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\bf {\textsc{64 GPUs}}}}} 
% Train     & 14.7     & 13.5		    & 14.4         & \bf 13.4  \\
% Novel      &  19.3      &     17.7      &   19.3     & \bf 16.7  \\
% All  &  17.0     &  15.6    &  16.9      & \bf 15.0\\
% \end{tabular}

% \begin{tabular}{rcccc}
% % \multicolumn{6}{c}{1.3B}
% \midrule
% \multicolumn{5}{l}{\bf 1.3B -- 128 GPUs -- 12k updates} \\
% \cmidrule{1-5}
% & \dense & \demix & \modular  & \densetomod \\
% & 1.3B & 7B & 10.4B & 10.4B \\
% \cmidrule{2-5}
% Train     &  14.2  &  13.7    &  13.3          & \bf 13.0  \\
% Novel      &    18.4    &    17.6       &    17.8    &  \bf 16.3 \\
% All  &    16.3     &   15.6  &  15.6     & \bf 14.6  \\
% \bottomrule \\
% \end{tabular}

\caption{\textbf{\delm{}s trained with \densetomod outperform all baselines across model scales}. \S\ref{subsection:core_results}: Average test-set perplexity ($\downarrow$) for each model scale (125M, 350M, 750M, 1.3B parameters) across the 8 training, 8 evaluation, and all 16 domains described in \S\ref{subsection:core_experimental_setup}. Total parameters are shown for each model type at each scale. At 125M parameter per GPU scale, we show the mean and standard deviation of results over 8 random seeds. For \densetomod, we display results with 50\% of compute dedicated to seed training. \demix outperforms \denselm. \delm{}s trained with \densetomod achieve the lowest average test perplexity on the 8 train as well as the 8 novel domains at all 4 model scales.  }

% , and \modular  outperforms \dense on the 8 train domains but does not generalize well. 
\label{tab:base_results}
\end{table}


==> tables/averaging_results_scaling.tex <==
% \begin{table*}[t]\small
% \centering
% % \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% &  \multicolumn{4}{c}{ \bf GPT-3 Small} \\
% \cmidrule{2-5}
% % % \emph{Shared Params}  & 124M & 124M & 96.1M & 67.8M  \\
% % % \emph{Expert Params}  & 0 & 0 & 28.3M & 56.7M  \\
% % % \emph{Total Params} & 124M & 124M & 322.8M & 521.1M  \\
% % \cmidrule{2-5}

% \textbf{Domain} & \bf \dataparallel  & \bf \domaintoken & \bf \plusmodelayers (L/2) & \bf \plusmodelayers (L) \\ %& \boldmath{\lnot}\textbf{\dapt}\\
% \midrule 

% \oneb 


% % 82.1
% & 14.6 & 14.2 & 14.3 & \bf 13.5  \\ %& 79.0$_{4.1}$\\


% \cs 
% % 82.1
% & 17.9 & 17.8 & 17.0 & \bf 15.6  \\ %& 79.0$_{4.1}$\\


% \legal 
% % 82.1
% & 10.5 & 10.1 &  9.5 & \bf 9.0   \\ %& 79.0$_{4.1}$\\


% \med  
% % 82.1
% & 13.8 & 14.1 & 13.4 & \bf 11.8 \\ %& 79.0$_{4.1}$\\


% \webtext 
% % 82.1
% & 22.0 & \bf 20.5 & 21.8 & 21.1 \\%& 79.0$_{4.1}$\\


% \realnews 
% % 82.1
% & 20.1 & \bf 18.6 & 20.0 &  18.8 \\ %& 79.0$_{4.1}$\\


% \reddit 
% % 82.1
% & 40.9 & \bf 40.3 & 41.6 &  40.8 \\ %& 79.0$_{4.1}$\\


% \reviews 
% % 82.1
% & 23.9 &  23.2 & 22.3 &  \bf 20.5\\ %& 79.0$_{4.1}$\\

% \midrule
% \bf Average & 20.5 & 19.9 &  20.0 & \bf 18.9 \\

% \bottomrule
% \end{tabular}
% % }
% \caption{Conditioning GPT-3 small on domains improves in-domain test performance, when training with 32 GPUs for 48 hours. See Appendix \label{sec:validation_curves} for validation curves during training.} 
% \label{tab:base_results}
% \end{table*}


\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rcccc}
\toprule
& \multicolumn{4}{c}{\bf \# training domains }\\
& 8 & 16 & 32 & 64 \\
% &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-5}


\bf \dense (350M)                  &  21.1   & 23.1 &  21.4  & 19.3\\
\bf \modular (350M; posterior weighted average)                  &  20.7  & 20.6 &  19.6  & 17.6 \\
\bf \modular (350M; posterior weights + greedy soup average)                  &  20.2   & 20.2 &  19.1  & 17.3 \\
\bf \dense (1.3B)                  & 18.5  & 19.2        &  18.1     & 16.3 \\

\bottomrule \\
% \bf \dense XL (6144 GPU hours)      &   &   &    &   & \\
% \cmidrule{2-4}
% \bf \demixdapt (\S\ref{sec:dapt_improving_indomain}) & 17.7 & 14.6 & 13.7 \\
% \bf \densedapt (\S\ref{sec:dapt_improving_indomain}) & 69.0 & 21.0 & 17.4 \\

%& \boldmath{\lnot}\textbf{\dapt}\\

%&\boldmath{\lnot}\textbf{\dapt}\\
% \bf \plusdomainparallel (Mixed) & \bf 17.6 & \bf 14.7 & \bf 13.9 \\ %& \boldmath{\lnot}\textbf{\dapt}\\

% \bottomrule
\end{tabular}

% }
\caption{Comparing \modular with expert averaging with the performance of \dense baselines on novel domains.Here we observe that expert averaging does not outperform output ensembling, but results in large gains in performance over dense models at a similar computational budget.}
\label{tab:averaging_results_scaling}
\end{table}


==> tables/big_dataset.tex <==
\begin{table*}[t]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{lllr}
\toprule
& \bf Domain & \bf Corpus &  \bf \# Train (Eval.) Tokens  \\
\midrule 

% \midrule[0.03em]




\parbox[t]{3pt}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\bf {\textsc{Training}}}}} & \oneb 
& 30M NewsWire sentences \citep{chelba2014billion} 
& 700M (10M) \\
& \cs 
& 1.89M full-text CS papers from S2ORC \citep{lo-wang-2020-s2orc} 
& 4.5B  (10M)\\
& \legal
& 2.22M U.S. court opinions \citep{caselaw2018} 
& 10.5B (10M) \\
 & \med      
& 3.2M full-text medical papers from  S2ORC \citep{lo-wang-2020-s2orc}  
& 9.5B (10M)\\

& \textsc{WebText}$^\dagger$
& 8M Web documents \citep{Gokaslan2019OpenWeb} 
& 6.5B  (10M)\\

% \midrule[0.03em]
& \textsc{RealNews}$^\dagger$
& 35M articles from \realnews  \cite{Zellers2019DefendingAN}%\footnote{similar to \ccnews sub-corpus used in \roberta pretraining}
& 15B (10M) \\
& \reddit
& Reddit comments from pushshift.io \citep{baumgartner2020pushshift} 
& 25B  (10M)\\

% \midrule[0.03em]
& \textsc{Reviews}$^\dagger$
& 30M Amazon product reviews \citep{ni-etal-2019-justifying} 
& 2.1B (10M) \\

\midrule
& & 
& \bf{Total} \hspace{2mm}  73.8B (80M) \\
\midrule
\end{tabular}

\begin{tabular}{lllr}
& \bf Domain & \bf  Corpus & \bf \# Train (Eval.) Tokens \\
\midrule

 \parbox[t]{3pt}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\bf \textsc{Novel \tim{Elsewhere this is called out-of-domain?}}}}} & \aclpapers & 1.5K NLP papers from ACL \citep{Dasigi2021ADO} & 1M (1M)  \\
 & \textsc{Breaking News}$^\dagger$ 
& 20K English news articles \citep{baly:2018:EMNLP2018}  & 11M (1M) \\

& \textsc{Contracts}$^\dagger$ & 500 commercial legal contracts \citep{hendrycks2021cuad} & 1.5M (1M) \\
& \cord 
& 400K COVID-19 research papers \citep{wang2020cord19} &  60M (10M) \\
& \textsc{Github}
& 230K public Github code  \citep{githubcode} & 200M (10M) \\
& \gutenberg      
& 3.2M copyright-expired books \citep{gutenberg} & 3B (10M) \\
% \midrule[0.03em]

& \textsc{Tweets}$^\dagger$ 
& 1M English tweets from 2013-2018 & 8M (1M)
\\


&  \textsc{Yelp Reviews}$^\dagger$ 
& 6M Yelp restaurant reviews \citep{yelpreviews} & 600M (10M)\\




\bottomrule
\end{tabular}

% }
\caption{Domains that make up our multi-domain training corpus, including the size of our training and evaluation (i.e. validation and test) data, in whitespace-separated tokens. We borrow these datasets from \citet{demix}.}
% \nascomment{should top row explain what's in parentheses (``Eval.'' like in the subheader for novel domains)?}}
\label{tab:datasets}
\end{table*}

==> tables/dense_ratios.tex <==
% \begin{table*}[t]\small
% \centering
% % \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% &  \multicolumn{4}{c}{ \bf GPT-3 Small} \\
% \cmidrule{2-5}
% % % \emph{Shared Params}  & 124M & 124M & 96.1M & 67.8M  \\
% % % \emph{Expert Params}  & 0 & 0 & 28.3M & 56.7M  \\
% % % \emph{Total Params} & 124M & 124M & 322.8M & 521.1M  \\
% % \cmidrule{2-5}

% \textbf{Domain} & \bf \dataparallel  & \bf \domaintoken & \bf \plusmodelayers (L/2) & \bf \plusmodelayers (L) \\ %& \boldmath{\lnot}\textbf{\dapt}\\
% \midrule 

% \oneb 


% % 82.1
% & 14.6 & 14.2 & 14.3 & \bf 13.5  \\ %& 79.0$_{4.1}$\\


% \cs 
% % 82.1
% & 17.9 & 17.8 & 17.0 & \bf 15.6  \\ %& 79.0$_{4.1}$\\


% \legal 
% % 82.1
% & 10.5 & 10.1 &  9.5 & \bf 9.0   \\ %& 79.0$_{4.1}$\\


% \med  
% % 82.1
% & 13.8 & 14.1 & 13.4 & \bf 11.8 \\ %& 79.0$_{4.1}$\\


% \webtext 
% % 82.1
% & 22.0 & \bf 20.5 & 21.8 & 21.1 \\%& 79.0$_{4.1}$\\


% \realnews 
% % 82.1
% & 20.1 & \bf 18.6 & 20.0 &  18.8 \\ %& 79.0$_{4.1}$\\


% \reddit 
% % 82.1
% & 40.9 & \bf 40.3 & 41.6 &  40.8 \\ %& 79.0$_{4.1}$\\


% \reviews 
% % 82.1
% & 23.9 &  23.2 & 22.3 &  \bf 20.5\\ %& 79.0$_{4.1}$\\

% \midrule
% \bf Average & 20.5 & 19.9 &  20.0 & \bf 18.9 \\

% \bottomrule
% \end{tabular}
% % }
% \caption{Conditioning GPT-3 small on domains improves in-domain test performance, when training with 32 GPUs for 48 hours. See Appendix \label{sec:validation_curves} for validation curves during training.} 
% \label{tab:base_results}
% \end{table*}



\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rccccccccccc}
\toprule
& \multicolumn{10}{c}{\bf Seed Phase (125M Parameter Model / Expert)}\\
& 0\% & 10\% & 20\% & 30\% & 40\% & 50\% & 60\% & 70\% & 80\% & 90\% & 100\%\\
\cmidrule{2-12}
\bf Train Domains    & 17.9 & 17.3 & \bf 17.1 & \bf 17.1 & 17.2     & 17.2 & 17.4 & 17.6       & 18.0 & 18.7 & 19.8 \\
\bf Eval Domains       & 23.8  & 23.7 & 23.0     & 22.8     & 22.7     & 22.7 & 22.5 & \bf 22.5   & 22.8 & 23.3 & 25.5  \\
\bf Avg                 & 20.9  & 20.5 & 20.1     & 20.0     & \bf 19.9 & 20.0 & 20.0 & 20.1       & 20.4 & 21.0 & 22.7\\

\midrule
\end{tabular}
% \vspace{4pt}
\begin{tabular}{rccccccccc}
% \toprule
& \multicolumn{9}{c}{\bf Seed Phase (350M Parameter Model / Expert)}\\
& 0\% & 12.5\% & 25\% & 37.5\% & 50\% & 62.5\% & 75\% & 87.5\% & 100\%\\
% &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-10}
\bf Train Domains & 15.3 & 15.0   & 14.9   & \bf 14.7   & \bf 14.7    & 14.9  & 15.2  & 15.7  & 16.3 \\
\bf Eval Domains & 21.3  & 20.0   & 19.6   & 19.0  & 18.6    & \bf 18.4  & 18.6   & 19.4   & 20.8 \\
\bf Avg & 18.3   & 17.5  & 17.2   & 16.9  & \bf 16.7    & \bf 16.7   & 16.9   & 17.5  & 18.5\\
\bottomrule \\
\end{tabular}
% \begin{tabular}{rccccccccccccccccc}
% \toprule
% & \multicolumn{13}{c}{\bf Dense Phase (350M Parameter Model / Experts)}\\
% % & 0\% & 10\% & 20\% & 30\% & 40\% & 50\% & 60\% & 70\% & 80\% & 90\% & 100\%\\
% % &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
% \cmidrule{2-16}
% \bf Training Domains & 15.3 & 15.1 & 15.0   & 14.8 & 14.9   & \bf 14.7  & \bf 14.7  & \bf 14.7  & \bf 14.7    & 14.8  & 14.9  & 15.0  & x  & 15.4  & 15.7  & 15.7 & 16.3 \\
% \bf Novel Domains & 21.3 & 20.9 & 20.0  & 19.7  & 19.6  & 19.2  & 19.0  & 18.7  & 18.6    & 18.5    & \bf 18.4  & 18.6  & x   & 19.2  & 19.4  & 19.4 & 20.8 \\
% \bf Avg & 18.3 & 18.0   & 17.5  & 17.3  & 17.2  & 17.0  & 16.9  & 16.7  & 16.7  & \bf 16.6    & 16.7  & 16.8  & x   & 17.3  & 17.5  & 17.6  & 18.5\\
% \bottomrule
% \end{tabular}

% }
\caption{Perplexity on in and out of domain test sets with different seed phase compute budgets for the 125M 350M parameter LMs. We observe optimal performance across all domains with roughly equal splits of seed and branched training.  }
\label{tab:dense_ratios}
\end{table}


==> tables/exp_setup.tex <==
% \begin{table*}[t]\small
% \centering
% % \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% &  \multicolumn{4}{c}{ \bf GPT-3 Small} \\
% \cmidrule{2-5}
% % % \emph{Shared Params}  & 124M & 124M & 96.1M & 67.8M  \\
% % % \emph{Expert Params}  & 0 & 0 & 28.3M & 56.7M  \\
% % % \emph{Total Params} & 124M & 124M & 322.8M & 521.1M  \\
% % \cmidrule{2-5}

% \textbf{Domain} & \bf \dataparallel  & \bf \domaintoken & \bf \plusmodelayers (L/2) & \bf \plusmodelayers (L) \\ %& \boldmath{\lnot}\textbf{\dapt}\\
% \midrule 

% \oneb 


% % 82.1
% & 14.6 & 14.2 & 14.3 & \bf 13.5  \\ %& 79.0$_{4.1}$\\


% \cs 
% % 82.1
% & 17.9 & 17.8 & 17.0 & \bf 15.6  \\ %& 79.0$_{4.1}$\\


% \legal 
% % 82.1
% & 10.5 & 10.1 &  9.5 & \bf 9.0   \\ %& 79.0$_{4.1}$\\


% \med  
% % 82.1
% & 13.8 & 14.1 & 13.4 & \bf 11.8 \\ %& 79.0$_{4.1}$\\


% \webtext 
% % 82.1
% & 22.0 & \bf 20.5 & 21.8 & 21.1 \\%& 79.0$_{4.1}$\\


% \realnews 
% % 82.1
% & 20.1 & \bf 18.6 & 20.0 &  18.8 \\ %& 79.0$_{4.1}$\\


% \reddit 
% % 82.1
% & 40.9 & \bf 40.3 & 41.6 &  40.8 \\ %& 79.0$_{4.1}$\\


% \reviews 
% % 82.1
% & 23.9 &  23.2 & 22.3 &  \bf 20.5\\ %& 79.0$_{4.1}$\\

% \midrule
% \bf Average & 20.5 & 19.9 &  20.0 & \bf 18.9 \\

% \bottomrule
% \end{tabular}
% % }
% \caption{Conditioning GPT-3 small on domains improves in-domain test performance, when training with 32 GPUs for 48 hours. See Appendix \label{sec:validation_curves} for validation curves during training.} 
% \label{tab:base_results}
% \end{table*}


\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{lrcccc}
\toprule
& & \multicolumn{4}{c}{\bf Parameters per GPU}\\
& & 125M & 350M & 760M & 1.3B \\
% &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{3-6}
\parbox[t]{0.7pt}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf {\textsc{\dense}}}}} & \bf GPUs  & 16 & 32 & 64 & 128\\
& \bf Total Experts & 0 & 0 & 0 & 0 \\
& \bf GPUs/expert & 0 & 0 & 0 & 0 \\
& \bf Total params & 125M & 350M & 760M & 1.3B \\
& \bf TFLOPs/update & 556 &  3279 & 13,637 & 23,250 \\
& \bf TFLOPs/GPU  & \bf{31} & \bf 37 & 45 & 51 \\
\cmidrule{3-6 }
\parbox[t]{0.7pt}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf {\textsc{\demix}}}}} & \bf GPUs  & 16 & 32 & 64 & 128\\
& \bf Total Experts & 8 & 8 & 8 & 8 \\
& \bf GPUs/expert & 2 & 4 & 8 & 16 \\
& \bf Total params & 512M & 1.8B & 3.8B & 7.0B \\
& \bf TFLOPs/update & 556 & 3279 & 13,637 & 23,250 \\
& \bf TFLOPs/GPU & \bf 31 & \bf 37 & \bf 48 & \bf 55 \\

% \cmidrule{2-4}
% \bf \demixdapt (\S\ref{sec:dapt_improving_indomain}) & 17.7 & 14.6 & 13.7 \\
% \bf \densedapt (\S\ref{sec:dapt_improving_indomain}) & 69.0 & 21.0 & 17.4 \\

%& \boldmath{\lnot}\textbf{\dapt}\\

%&\boldmath{\lnot}\textbf{\dapt}\\
% \bf \plusdomainparallel (Mixed) & \bf 17.6 & \bf 14.7 & \bf 13.9 \\ %& \boldmath{\lnot}\textbf{\dapt}\\

\bottomrule \\
\end{tabular}

% }
\caption{Our specifications for training \dense and \demix LMs. All models are trained for about 48 hours on V100 GPUs. \demixlayers increase the total parameters of the LM while maintaining (or increasing) throughput, measured in TFLOPs/GPU. We use the formula described in \citet{narayanan2021efficient} to calculate these metrics. See \S\ref{sec:tflops} for more details.}
\label{tab:exp_setup}
\end{table}


==> tables/expert_removal_alt.tex <==
\begin{table}[t]\small
\centering

\begin{tabular}{lrrcc}
\toprule
% & & \multicolumn{2}{r}{\bf Avg Test PPL} \\
% & & & \multicolumn{2}{r}{\bf(PPL $\Delta$)} \\
% \cmidrule{1-5} 
&& &  \thead{+ Expert \\  (Average Test PPL $\downarrow$)} & \thead{--Expert  \\ ($\Delta$ PPL) }\\
\midrule
&& \bf 8 train domains & 17.2 & (+9.4) \\
\midrule
\parbox[t]{1pt}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{seed}}}} &
\parbox[t]{1pt}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{corpus}}}} &
 \bf Wikipedia & 17.7 & (+11.9)\\
&& \bf C4       & 17.9 & (+11.8)\\
&& \bf StackOverflow  & 18.4 & (+12.7) \\
&& \bf JavaScript  & 19.2 & (+13.6) \\
% \vspace{0.01mm} \\
\bottomrule \\
\end{tabular}

\caption{\textbf{The ability to reduce the influence of domains through \dslm removal is (mostly) robust to seed training corpus}. \S\ref{subsection:dense_phase_corpus}: We present the average test perplexity for the 8 train domains in \delm{}s where all \dslm{}s are active. We vary the seed training corpora. In parentheses, we show the \emph{increase} in perplexity when the \dslm trained to specialize on each test domain is removed at inference time. High increases are desired, as they suggest the ease of removing data from the \delm{}'s distribution after training has completed.}
\label{tab:expert_removal}
\end{table}

==> tables/full_base_results.tex <==
\begin{table}[t]\small
\centering
% \begin{subtable}[t]{0.3\textwidth}
% \begin{tabular}{rcccc}
% \toprule
% \multicolumn{5}{l}{\bf 125M -- 16 GPUs -- 80k updates} \\
% \cmidrule{1-5}
% & \dense & \demix & \modular  & \densetomod \\
% & 125M & 512M & 1B  & 1B \\
% \cmidrule{2-5}
% Train     & 19.8      & 17.7     & 17.9          & \bf 17.2 \\
% Novel      &  25.6       &   23.1         &    23.8   & \bf 22.7 \\
% All  &   22.7    & 20.4      & 20.9     & \bf 20.0 \\
% \bottomrule
% \end{tabular}
% % \end{subtable}

% % \begin{subtable}[t]{0.3\textwidth}
% \begin{tabular}{rcccc}
% % \multicolumn{5}{c}{350M}
% \toprule
% \multicolumn{5}{l}{\bf 350M -- 32 GPUs -- 32k updates} \\
% \cmidrule{1-5}
% & \dense & \demix & \modular  & \densetomod \\
% & 350M & 1.8B & 2.8B  & 2.8B \\
% \cmidrule{2-5}
% Train     &  16.3    &   15.0  &  15.3         &  \bf 14.7 \\
% Novel      &  20.8      &     19.9      &    21.3      & \bf 18.6\\
% All      & 18.5    &    17.5  &  18.3     &  \bf 16.7 \\
% \bottomrule
% \end{tabular}
% % \end{subtable}

% \begin{tabular}{rcccc}
% % \multicolumn{5}{c}{750M}
% \toprule
% \multicolumn{5}{l}{\bf 750M -- 64 GPUs -- 24k updates} \\
% \cmidrule{1-5}
% & \dense & \demix & \modular  & \dense to \modular \\
% & 750M & 3.8B  & 6B  & 6B \\
% \cmidrule{2-5}
% % \parbox[t]{3pt}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\bf {\textsc{750M}}}}} &
% % \parbox[t]{3pt}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\bf {\textsc{64 GPUs}}}}} 
% Train     & 14.7     & 13.5		    & 14.4         & \bf 13.4  \\
% Novel      &  19.3      &     17.7      &   19.3     & \bf 16.7  \\
% All  &  17.0     &  15.6    &  16.9      & \bf 15.0\\
% \bottomrule
% \end{tabular}

% \begin{tabular}{rcccc}
% % \multicolumn{6}{c}{1.3B}
% \toprule
% \multicolumn{5}{l}{\bf 1.3B -- 128 GPUs -- 12k updates} \\
% \cmidrule{1-5}
% & \dense & \demix & \modular  & \dense to \modular \\
% & 1.3B & 7B & 10.4B & 10.4B \\
% \cmidrule{2-5}
% Train     &  14.2  &  13.7    &  13.3          & \bf 13.0  \\
% Novel      &    18.4    &    17.6       &    17.8    &  \bf 16.3 \\
% All  &    16.3     &   15.6  &  15.6     & \bf 14.6  \\
% \bottomrule \\
% \end{tabular}

% \begin{subtable}[t]{0.3\textwidth}
\begin{tabular}{rcccccc}
\toprule
\multicolumn{7}{l}{\bf 125M -- 16 GPUs -- 80k updates} \\
\cmidrule{1-7}
& & Unbalanced & & & Random & \\
& \dense & \dense & \demix & \modular & \densetomod & \densetomod \\
& 125M & 125M & 512M & 1B & 1B & 1B \\
\cmidrule{2-7}
Train   & 19.8  & 20.7  & 17.7  & 17.9  & 23.0  & \bf 17.2 \\
Novel   & 25.6  & 26.4  & 23.1  & 23.8  & 26.0  & \bf 22.7 \\
All     & 22.7  & 23.5  & 20.4  & 20.9  & 24.7  & \bf 20.0 \\
\bottomrule
\end{tabular}
% \end{subtable}

% \begin{subtable}[t]{0.3\textwidth}
\begin{tabular}{rcccccc}
\toprule
\multicolumn{7}{l}{\bf 350M -- 32 GPUs -- 32k updates} \\\cmidrule{1-7}
& & Unbalanced & & & Random & \\ 
& \dense & \dense & \demix & \modular & \densetomod & \densetomod \\
& 350M & 350M & 1.8B & 2.8B & 2.8B & 2.8B \\
\cmidrule{2-7}
Train   & 16.3  & 16.7  & 15.0  & 15.3  & & \bf 14.7 \\
Novel   & 20.8  & 21.2  & 19.9  & 21.3  & & \bf 18.6 \\
All     & 18.5  & 19.0  & 17.5  & 18.3  & & \bf 16.7 \\
\bottomrule
\end{tabular}

\begin{tabular}{rcccccc}
\toprule
\multicolumn{7}{l}{\bf 750M -- 64 GPUs -- 24k updates} \\ \cmidrule{1-7}
& & Unbalanced & & & Random & \\ 
& \dense & \dense & \demix & \modular & \densetomod & \densetomod \\
& 750M & 750M & 3.8B & 6B & 6B & 6B \\
\cmidrule{2-7}
Train   & 14.7  & 14.9  & 13.5  & 14.4  &   & \bf 13.4 \\
Novel   & 19.3  & 19.8  & 17.7  & 19.3  &   & \bf 16.7 \\
All     & 17.0  & 17.4  & 15.6  & 16.9  &   & \bf 15.0 \\
\bottomrule
\end{tabular}

\begin{tabular}{rcccccc}
\toprule
\multicolumn{5}{l}{\bf 1.3B -- 128 GPUs -- 12k updates} \\ \cmidrule{1-7}
& & Unbalanced & & & Random & \\ 
& \dense & \dense & \demix & \modular & \densetomod & \densetomod \\
& 1.3B & 1.3B & 7B & 10.4B & 10.4B & 10.4B \\
\cmidrule{2-7}
Train   &  14.2 & 15.0  & 13.7  & 13.3  &   & \bf 13.0 \\
Novel   &  18.4 & 19.5  & 17.6  & 17.8  &   & \bf 16.3 \\
All     &  16.3 & 17.3  & 15.6  & 15.6  &   & \bf 14.6 \\
\bottomrule \\
\end{tabular}
\caption{Average test-set perplexity ($\downarrow$) for each model scale (125M, 350M, 750M, 1.3B parameters) across the 8 training, 8 novel, and all 16 domains. Total compute budget (in update numbers) and GPU usage counts are shown for each model size, and total parameters are shown for each model type at each size. For \dense to \modular, we display results with 50\% dense training. \demix outperforms \dense, and \modular  outperforms \dense on the 8 train domains but does not generalize well. \dense to \modular achieves the lowest average test perplexity on the 8 train as well as the 8 novel domains at all 4 model scales.}
\label{tab:base_results}
\end{table}

==> tables/gpu_hours.tex <==
% \begin{table*}[t]\small
% \centering
% % \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% &  \multicolumn{4}{c}{ \bf GPT-3 Small} \\
% \cmidrule{2-5}
% % % \emph{Shared Params}  & 124M & 124M & 96.1M & 67.8M  \\
% % % \emph{Expert Params}  & 0 & 0 & 28.3M & 56.7M  \\
% % % \emph{Total Params} & 124M & 124M & 322.8M & 521.1M  \\
% % \cmidrule{2-5}

% \textbf{Domain} & \bf \dataparallel  & \bf \domaintoken & \bf \plusmodelayers (L/2) & \bf \plusmodelayers (L) \\ %& \boldmath{\lnot}\textbf{\dapt}\\
% \midrule 

% \oneb 


% % 82.1
% & 14.6 & 14.2 & 14.3 & \bf 13.5  \\ %& 79.0$_{4.1}$\\


% \cs 
% % 82.1
% & 17.9 & 17.8 & 17.0 & \bf 15.6  \\ %& 79.0$_{4.1}$\\


% \legal 
% % 82.1
% & 10.5 & 10.1 &  9.5 & \bf 9.0   \\ %& 79.0$_{4.1}$\\


% \med  
% % 82.1
% & 13.8 & 14.1 & 13.4 & \bf 11.8 \\ %& 79.0$_{4.1}$\\


% \webtext 
% % 82.1
% & 22.0 & \bf 20.5 & 21.8 & 21.1 \\%& 79.0$_{4.1}$\\


% \realnews 
% % 82.1
% & 20.1 & \bf 18.6 & 20.0 &  18.8 \\ %& 79.0$_{4.1}$\\


% \reddit 
% % 82.1
% & 40.9 & \bf 40.3 & 41.6 &  40.8 \\ %& 79.0$_{4.1}$\\


% \reviews 
% % 82.1
% & 23.9 &  23.2 & 22.3 &  \bf 20.5\\ %& 79.0$_{4.1}$\\

% \midrule
% \bf Average & 20.5 & 19.9 &  20.0 & \bf 18.9 \\

% \bottomrule
% \end{tabular}
% % }
% \caption{Conditioning GPT-3 small on domains improves in-domain test performance, when training with 32 GPUs for 48 hours. See Appendix \label{sec:validation_curves} for validation curves during training.} 
% \label{tab:base_results}
% \end{table*}


\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rcccc}
\toprule
& \multicolumn{4}{c}{\bf \# training domains }\\
& 8 & 16 & 32 & 64 \\
% &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-5}


\bf \dense \& \modular (125M)                  & 768 & 928          &  1088    & 1328\\
\bf \dense \& \modular (350M) & 1536 &    1856   &  2496   & 2656\\
\bf \dense 1.3B  & 6144 & 6144    &  6144    & 6144 \\

\bottomrule \\
% \bf \dense XL (6144 GPU hours)      &   &   &    &   & \\
% \cmidrule{2-4}
% \bf \demixdapt (\S\ref{sec:dapt_improving_indomain}) & 17.7 & 14.6 & 13.7 \\
% \bf \densedapt (\S\ref{sec:dapt_improving_indomain}) & 69.0 & 21.0 & 17.4 \\

%& \boldmath{\lnot}\textbf{\dapt}\\

%&\boldmath{\lnot}\textbf{\dapt}\\
% \bf \plusdomainparallel (Mixed) & \bf 17.6 & \bf 14.7 & \bf 13.9 \\ %& \boldmath{\lnot}\textbf{\dapt}\\

% \bottomrule
\end{tabular}

% }
\caption{GPU hours for each setting we compare in \S\ref{sec:scaling_domains}. We train the \dense 1.3B parameter model for 2 days on 128 GPUs with each training dataset. We compare to \modular scaled into the same dataset, and \dense model matching in total number of parameters per GPU and total GPU hours. }
\label{tab:scaling_results}
\end{table}


==> tables/in_domain_scaling_results.tex <==
% \begin{table*}[t]\small
% \centering
% % \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% &  \multicolumn{4}{c}{ \bf GPT-3 Small} \\
% \cmidrule{2-5}
% % % \emph{Shared Params}  & 124M & 124M & 96.1M & 67.8M  \\
% % % \emph{Expert Params}  & 0 & 0 & 28.3M & 56.7M  \\
% % % \emph{Total Params} & 124M & 124M & 322.8M & 521.1M  \\
% % \cmidrule{2-5}

% \textbf{Domain} & \bf \dataparallel  & \bf \domaintoken & \bf \plusmodelayers (L/2) & \bf \plusmodelayers (L) \\ %& \boldmath{\lnot}\textbf{\dapt}\\
% \midrule 

% \oneb 


% % 82.1
% & 14.6 & 14.2 & 14.3 & \bf 13.5  \\ %& 79.0$_{4.1}$\\


% \cs 
% % 82.1
% & 17.9 & 17.8 & 17.0 & \bf 15.6  \\ %& 79.0$_{4.1}$\\


% \legal 
% % 82.1
% & 10.5 & 10.1 &  9.5 & \bf 9.0   \\ %& 79.0$_{4.1}$\\


% \med  
% % 82.1
% & 13.8 & 14.1 & 13.4 & \bf 11.8 \\ %& 79.0$_{4.1}$\\


% \webtext 
% % 82.1
% & 22.0 & \bf 20.5 & 21.8 & 21.1 \\%& 79.0$_{4.1}$\\


% \realnews 
% % 82.1
% & 20.1 & \bf 18.6 & 20.0 &  18.8 \\ %& 79.0$_{4.1}$\\


% \reddit 
% % 82.1
% & 40.9 & \bf 40.3 & 41.6 &  40.8 \\ %& 79.0$_{4.1}$\\


% \reviews 
% % 82.1
% & 23.9 &  23.2 & 22.3 &  \bf 20.5\\ %& 79.0$_{4.1}$\\

% \midrule
% \bf Average & 20.5 & 19.9 &  20.0 & \bf 18.9 \\

% \bottomrule
% \end{tabular}
% % }
% \caption{Conditioning GPT-3 small on domains improves in-domain test performance, when training with 32 GPUs for 48 hours. See Appendix \label{sec:validation_curves} for validation curves during training.} 
% \label{tab:base_results}
% \end{table*}


\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rcccc}
\toprule
& \multicolumn{4}{c}{\bf \# training domains }\\
& 8 & 16 & 32 & 64 \\
% &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-5}


\bf \modular (125M)                  &   17.9   & 17.9 &    17.9    & 17.9 \\
\bf \modular (350M)                  &  15.1   & 15.1 &  15.1   & 15.1 \\
\bf \dense (1.3B)                  & 14.8 & 15.2         &  16.0   & 16.3 \\

\bottomrule \\
% \bf \dense XL (6144 GPU hours)      &   &   &    &   & \\
% \cmidrule{2-4}
% \bf \demixdapt (\S\ref{sec:dapt_improving_indomain}) & 17.7 & 14.6 & 13.7 \\
% \bf \densedapt (\S\ref{sec:dapt_improving_indomain}) & 69.0 & 21.0 & 17.4 \\

%& \boldmath{\lnot}\textbf{\dapt}\\

%&\boldmath{\lnot}\textbf{\dapt}\\
% \bf \plusdomainparallel (Mixed) & \bf 17.6 & \bf 14.7 & \bf 13.9 \\ %& \boldmath{\lnot}\textbf{\dapt}\\

% \bottomrule
\end{tabular}

% }
\caption{Average perplexity on \textbf{the first eight domains (G1)} as you increase the number of domains in the training data. We observe progressively degrading performance in dense models on G1 domains. performance on G1 stays static in \modular models. }
\label{tab:scaling_results}
\end{table}


==> tables/novel_domain_scaling_results.tex <==
% \begin{table*}[t]\small
% \centering
% % \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% &  \multicolumn{4}{c}{ \bf GPT-3 Small} \\
% \cmidrule{2-5}
% % % \emph{Shared Params}  & 124M & 124M & 96.1M & 67.8M  \\
% % % \emph{Expert Params}  & 0 & 0 & 28.3M & 56.7M  \\
% % % \emph{Total Params} & 124M & 124M & 322.8M & 521.1M  \\
% % \cmidrule{2-5}

% \textbf{Domain} & \bf \dataparallel  & \bf \domaintoken & \bf \plusmodelayers (L/2) & \bf \plusmodelayers (L) \\ %& \boldmath{\lnot}\textbf{\dapt}\\
% \midrule 

% \oneb 


% % 82.1
% & 14.6 & 14.2 & 14.3 & \bf 13.5  \\ %& 79.0$_{4.1}$\\


% \cs 
% % 82.1
% & 17.9 & 17.8 & 17.0 & \bf 15.6  \\ %& 79.0$_{4.1}$\\


% \legal 
% % 82.1
% & 10.5 & 10.1 &  9.5 & \bf 9.0   \\ %& 79.0$_{4.1}$\\


% \med  
% % 82.1
% & 13.8 & 14.1 & 13.4 & \bf 11.8 \\ %& 79.0$_{4.1}$\\


% \webtext 
% % 82.1
% & 22.0 & \bf 20.5 & 21.8 & 21.1 \\%& 79.0$_{4.1}$\\


% \realnews 
% % 82.1
% & 20.1 & \bf 18.6 & 20.0 &  18.8 \\ %& 79.0$_{4.1}$\\


% \reddit 
% % 82.1
% & 40.9 & \bf 40.3 & 41.6 &  40.8 \\ %& 79.0$_{4.1}$\\


% \reviews 
% % 82.1
% & 23.9 &  23.2 & 22.3 &  \bf 20.5\\ %& 79.0$_{4.1}$\\

% \midrule
% \bf Average & 20.5 & 19.9 &  20.0 & \bf 18.9 \\

% \bottomrule
% \end{tabular}
% % }
% \caption{Conditioning GPT-3 small on domains improves in-domain test performance, when training with 32 GPUs for 48 hours. See Appendix \label{sec:validation_curves} for validation curves during training.} 
% \label{tab:base_results}
% \end{table*}


\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rcccc}
\toprule
& \multicolumn{4}{c}{\bf \# training domains }\\
& 8 & 16 & 32 & 64 \\
% &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-5}


\bf \modular (125M)                  &   23.6   & 23.4 &    22.0    & 20.0 \\
\bf \modular (350M)                  &  19.4   & 19.3 &  18.2  & 16.7 \\
\bf \modular (350M)                  &  19.4   & 19.3 &  18.2  & 16.7 \\

\bf \dense (1.3B)                  & 18.5  & 19.2        &  18.1     & 16.3 \\

\bottomrule \\
% \bf \dense XL (6144 GPU hours)      &   &   &    &   & \\
% \cmidrule{2-4}
% \bf \demixdapt (\S\ref{sec:dapt_improving_indomain}) & 17.7 & 14.6 & 13.7 \\
% \bf \densedapt (\S\ref{sec:dapt_improving_indomain}) & 69.0 & 21.0 & 17.4 \\

%& \boldmath{\lnot}\textbf{\dapt}\\

%&\boldmath{\lnot}\textbf{\dapt}\\
% \bf \plusdomainparallel (Mixed) & \bf 17.6 & \bf 14.7 & \bf 13.9 \\ %& \boldmath{\lnot}\textbf{\dapt}\\

% \bottomrule
\end{tabular}

% }
\caption{\modular approaches the performance of \dense 1.3B on the novel domains.}
\label{tab:scaling_results}
\end{table}


==> tables/scaling_datasets_main.tex <==
\begin{table}[t]
\tiny

\caption*{\textsc{96-domain corpus (XX whitespace tokens)}} 
\vspace{2mm}
\begin{subtable}[t]{0.24\textwidth}


\begin{tabular}{lr}
% \multicolumn{2}{c}{\bf Research} & 
\midrule
 \bf Domain  &  \bf\# Train Tokens  \\
\midrule 


Reddit
& 700M  \\
Legal
& 6.5B  \\


Medicine
& 15B  \\
 \reddit
& 25B  \\


C4
& 2.1B  \\

RealNews
 & 600M \\

 Biology
 & 600M \\

Stories
 & 600M \\

JavaScript
 & 600M \\
Java 
 & 600M \\
OpenWebText
 & 600M \\
  \textsc{CS} 
 & 600M \\



























































































































































\midrule
\end{tabular}
\end{subtable}
\begin{subtable}[t]{0.24\textwidth}


\begin{tabular}{lr}
% \multicolumn{2}{c}{\bf Resesarch} & 
\midrule
 \bf Domain  &  \bf\# Train Tokens  \\
\midrule 




Physics
 & 600M \\

  HTML
 & 600M \\

 \textsc{C} 
 & 600M \\
\textsc{Math} & 600M \\
Book Reviews
 & 600M \\
C++
 & 600M \\
StackOverflow
 & 600M \\
Gutenberg 
 & 600M \\
  \textsc{Python} 
 & 600M \\
Wikipedia 
 & 600M \\
Unlabeled S2ORC
 & 600M \\
 DUMMY & 600M \\
    




























































































































































\midrule
\end{tabular}
\end{subtable}
\begin{subtable}[t]{0.24\textwidth}


\begin{tabular}{lr}
% \multicolumn{2}{c}{\bf Github Code} & 
\midrule
 \bf Domain  &  \bf\# Train Tokens  \\
\midrule 


C\# 
& 700M  \\
 Psychology 
& 4.5B  \\
 PHP
& 10.5B  \\
 Amazon Reviews     
& 9.5B \\
Markdown
& 6.5B  \\


Chemistry
& 15B  \\
Code Contests
& 25B  \\


Go
& 2.1B  \\

Twitter
& 600M \\

Economics
& 600M \\

StackExchange
& 600M \\

DM Mathematics
& 600M \\





























































































































































\midrule
\end{tabular}
\end{subtable}
\begin{subtable}[t]{0.24\textwidth}


\begin{tabular}{lr}
% \multicolumn{2}{c}{\bf Github Code} & 
\midrule
 \bf Domain  &  \bf\# Train Tokens  \\
\midrule 


CSS
& 700M  \\
Engineering
& 4.5B  \\
CORD19
& 10.5B  \\
Electronics
& 9.5B \\
Materials	
& 6.5B  \\


Geology	& 15B  \\
 \reddit
& 25B  \\


WMT Newscrawl & 2.1B  \\

Sociology & 600M \\

Clothing Reviews & 600M \\

Ruby & 600M \\

HackerNews & 600M \\




























































































































































\midrule
\end{tabular}
\end{subtable}
\hfill
\begin{subtable}[t]{0.24\textwidth}


\begin{tabular}{lr}
% \multicolumn{2}{c}{\bf Web Dumps} & 
\midrule
 \bf Domain  &  \bf\# Train Tokens  \\
\midrule 


Home Reviews
& 700M  \\
BookCorpus
& 4.5B  \\
OpenSubtitles	
& 10.5B  \\
1B
& 9.5B \\
Business & 6.5B  \\
Yelp Reviews & 700M  \\
Sports Reviews
& 4.5B  \\
Movie Reviews
& 10.5B  \\
Poli. Sci.      
& 9.5B \\
Geography & 6.5B  \\


Environment & 15B  \\


USPTO
& 2.1B  \\

















































































































































































\midrule
\end{tabular}
\end{subtable}
\begin{subtable}[t]{0.24\textwidth}


\begin{tabular}{lr}
% \multicolumn{2}{c}{\bf Books} & 
\midrule
 \bf Domain  &  \bf\# Train Tokens  \\
\midrule 
History & 600M \\
Gaming Reddit & 600M \\
Philosophy & 600M\\
ACL  &  600M\\
Sports Reddit & 600M\\
SCOTUS & 600M\\
Art Papers & 600M\\
Covid Tweets & 600M\\
PR Case Law & 600M\\
Movie plots & 600M\\
pcgaming & 600M\\
COHA (Mag.) & 600M\\ 











































































































































































\midrule
\end{tabular}
\end{subtable}
\begin{subtable}[t]{0.24\textwidth}


\begin{tabular}{lr}
% \multicolumn{2}{c}{\bf Code} & 
\midrule
 \bf Domain  &  \bf\# Train Tokens  \\
\midrule 


COHA (Fic.)
& 700M  \\
india
& 4.5B  \\
COHA (NonFic.)
& 10.5B  \\
 COHA (News)      
& 9.5B \\
TOEFL & 6.5B  \\


Arts Reviews
& 15B  \\
Blogs
& 25B  \\


Game Reviews
& 2.1B  \\

smashbros & 600M \\

nba & 600M \\

PeerRead & 600M \\

FORTRAN & 600M \\




























































































































































\midrule
\end{tabular}
\end{subtable}
\begin{subtable}[t]{0.24\textwidth}


\begin{tabular}{lr}
% \multicolumn{2}{c}{\bf Code} & 
\midrule
 \bf Domain  &  \bf\# Train Tokens  \\
\midrule 


TeX & 700M  \\
Perl & 4.5B  \\
Rust & 10.5B  \\
SQL & 9.5B \\
Congress Bills & 6.5B  \\


Enron & 15B  \\
PM Speeches & 25B  \\


cscareerquestions
& 2.1B  \\

financialindependence & 600M \\

Legal Contracts & 600M \\

RCT-20K  & 600M \\

explainlikeimfive & 600M \\




























































































































































\midrule
\end{tabular}
\end{subtable}
\caption{Domains that make up our 96-domain corpus, ordered by size}

\label{tab:scaling_datasets}
\end{table}


==> tables/scaling_results.tex <==
% \begin{table*}[t]\small
% \centering
% % \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% &  \multicolumn{4}{c}{ \bf GPT-3 Small} \\
% \cmidrule{2-5}
% % % \emph{Shared Params}  & 124M & 124M & 96.1M & 67.8M  \\
% % % \emph{Expert Params}  & 0 & 0 & 28.3M & 56.7M  \\
% % % \emph{Total Params} & 124M & 124M & 322.8M & 521.1M  \\
% % \cmidrule{2-5}

% \textbf{Domain} & \bf \dataparallel  & \bf \domaintoken & \bf \plusmodelayers (L/2) & \bf \plusmodelayers (L) \\ %& \boldmath{\lnot}\textbf{\dapt}\\
% \midrule 

% \oneb 


% % 82.1
% & 14.6 & 14.2 & 14.3 & \bf 13.5  \\ %& 79.0$_{4.1}$\\


% \cs 
% % 82.1
% & 17.9 & 17.8 & 17.0 & \bf 15.6  \\ %& 79.0$_{4.1}$\\


% \legal 
% % 82.1
% & 10.5 & 10.1 &  9.5 & \bf 9.0   \\ %& 79.0$_{4.1}$\\


% \med  
% % 82.1
% & 13.8 & 14.1 & 13.4 & \bf 11.8 \\ %& 79.0$_{4.1}$\\


% \webtext 
% % 82.1
% & 22.0 & \bf 20.5 & 21.8 & 21.1 \\%& 79.0$_{4.1}$\\


% \realnews 
% % 82.1
% & 20.1 & \bf 18.6 & 20.0 &  18.8 \\ %& 79.0$_{4.1}$\\


% \reddit 
% % 82.1
% & 40.9 & \bf 40.3 & 41.6 &  40.8 \\ %& 79.0$_{4.1}$\\


% \reviews 
% % 82.1
% & 23.9 &  23.2 & 22.3 &  \bf 20.5\\ %& 79.0$_{4.1}$\\

% \midrule
% \bf Average & 20.5 & 19.9 &  20.0 & \bf 18.9 \\

% \bottomrule
% \end{tabular}
% % }
% \caption{Conditioning GPT-3 small on domains improves in-domain test performance, when training with 32 GPUs for 48 hours. See Appendix \label{sec:validation_curves} for validation curves during training.} 
% \label{tab:base_results}
% \end{table*}


\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rcccc}
\toprule
& \multicolumn{4}{c}{\bf \# training domains }\\
& 8 & 16 & 32 & 64 \\
% &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-5}


\bf \dense (125M, compute matched)                  & 22.7 & 23.6          &  21.0     & 20.2\\
\bf \modular (125M)                  &  \bf 20.6   & \bf 20.1 &  \bf  17.7    & \bf 15.9 \\
\midrule
\bf \dense (350M, compute matched) & 18.4 &    19.4   &  17.2   & 15.6\\
\bf \modular (350M) & \bf 16.9 & \bf  16.5    &  \bf 14.9    & \bf 13.3 \\

\bottomrule \\
% \bf \dense XL (6144 GPU hours)      &   &   &    &   & \\
% \cmidrule{2-4}
% \bf \demixdapt (\S\ref{sec:dapt_improving_indomain}) & 17.7 & 14.6 & 13.7 \\
% \bf \densedapt (\S\ref{sec:dapt_improving_indomain}) & 69.0 & 21.0 & 17.4 \\

%& \boldmath{\lnot}\textbf{\dapt}\\

%&\boldmath{\lnot}\textbf{\dapt}\\
% \bf \plusdomainparallel (Mixed) & \bf 17.6 & \bf 14.7 & \bf 13.9 \\ %& \boldmath{\lnot}\textbf{\dapt}\\

% \bottomrule
\end{tabular}

% }
\caption{Average perplexity across all 96 domains as you increase the number of domains in training data. \modular guarantees monotonically improving performance as the number of domains increase, while \dense scaling makes no such guarantees. }
\label{tab:scaling_results}
\end{table}


==> tables/xl_comparison.tex <==
% \begin{table*}[t]\small
% \centering
% % \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% &  \multicolumn{4}{c}{ \bf GPT-3 Small} \\
% \cmidrule{2-5}
% % % \emph{Shared Params}  & 124M & 124M & 96.1M & 67.8M  \\
% % % \emph{Expert Params}  & 0 & 0 & 28.3M & 56.7M  \\
% % % \emph{Total Params} & 124M & 124M & 322.8M & 521.1M  \\
% % \cmidrule{2-5}

% \textbf{Domain} & \bf \dataparallel  & \bf \domaintoken & \bf \plusmodelayers (L/2) & \bf \plusmodelayers (L) \\ %& \boldmath{\lnot}\textbf{\dapt}\\
% \midrule 

% \oneb 


% % 82.1
% & 14.6 & 14.2 & 14.3 & \bf 13.5  \\ %& 79.0$_{4.1}$\\


% \cs 
% % 82.1
% & 17.9 & 17.8 & 17.0 & \bf 15.6  \\ %& 79.0$_{4.1}$\\


% \legal 
% % 82.1
% & 10.5 & 10.1 &  9.5 & \bf 9.0   \\ %& 79.0$_{4.1}$\\


% \med  
% % 82.1
% & 13.8 & 14.1 & 13.4 & \bf 11.8 \\ %& 79.0$_{4.1}$\\


% \webtext 
% % 82.1
% & 22.0 & \bf 20.5 & 21.8 & 21.1 \\%& 79.0$_{4.1}$\\


% \realnews 
% % 82.1
% & 20.1 & \bf 18.6 & 20.0 &  18.8 \\ %& 79.0$_{4.1}$\\


% \reddit 
% % 82.1
% & 40.9 & \bf 40.3 & 41.6 &  40.8 \\ %& 79.0$_{4.1}$\\


% \reviews 
% % 82.1
% & 23.9 &  23.2 & 22.3 &  \bf 20.5\\ %& 79.0$_{4.1}$\\

% \midrule
% \bf Average & 20.5 & 19.9 &  20.0 & \bf 18.9 \\

% \bottomrule
% \end{tabular}
% % }
% \caption{Conditioning GPT-3 small on domains improves in-domain test performance, when training with 32 GPUs for 48 hours. See Appendix \label{sec:validation_curves} for validation curves during training.} 
% \label{tab:base_results}
% \end{table*}


\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rcccc}
\toprule
& \multicolumn{4}{c}{\bf \# training domains }\\
& 8 & 16 & 32 & 64 \\
% &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-5}


\bf \modular (125M)                  &   20.6   & 20.1 &    17.7    & 15.9 \\
\bf \modular (350M)                  &  16.9   & 16.5 &  14.9   & 13.3 \\
\bf \dense (1.3B)                  & 16.0 & 16.0         &  14.6     & 13.1 \\

\bottomrule \\
% \bf \dense XL (6144 GPU hours)      &   &   &    &   & \\
% \cmidrule{2-4}
% \bf \demixdapt (\S\ref{sec:dapt_improving_indomain}) & 17.7 & 14.6 & 13.7 \\
% \bf \densedapt (\S\ref{sec:dapt_improving_indomain}) & 69.0 & 21.0 & 17.4 \\

%& \boldmath{\lnot}\textbf{\dapt}\\

%&\boldmath{\lnot}\textbf{\dapt}\\
% \bf \plusdomainparallel (Mixed) & \bf 17.6 & \bf 14.7 & \bf 13.9 \\ %& \boldmath{\lnot}\textbf{\dapt}\\

% \bottomrule
\end{tabular}

% }
\caption{Average perplexity across all 96 domains as you increase the number of domains in training data. With 64 domains, \modular (350M) approaches the overall performance of GPT-3 XL, with about 40\% of the total compute. }
\label{tab:scaling_results}
\end{table}

